Convergence of de Finetti's mixing measure in latent structure models for observed exchangeable sequences

Mixtures of product distributions are a powerful device for learning about heterogeneity within data populations. In this class of latent structure models, de Finetti's mixing measure plays the central role for describing the uncertainty about the latent parameters representing heterogeneity. In this paper posterior contraction theorems for de Finetti's mixing measure arising from finite mixtures of product distributions will be established, under the setting the number of exchangeable sequences of observed variables increases while sequence length(s) may be either fixed or varied. The role of both the number of sequences and the sequence lengths will be carefully examined. In order to obtain concrete rates of convergence, a first-order identifiability theory for finite mixture models and a family of sharp inverse bounds for mixtures of product distributions will be developed via a harmonic analysis of such latent structure models. This theory is applicable to broad classes of probability kernels composing the mixture model of product distributions for both continuous and discrete domain $\mathfrak{X}$. Examples of interest include the case the probability kernel is only weakly identifiable in the sense of Ho and Nguyen (2016), the case where the kernel is itself a mixture distribution as in hierarchical models, and the case the kernel may not have a density with respect to a dominating measure on an abstract domain $\mathfrak{X}$ such as Dirichlet processes.

==> deleted.tex <==
As is discussed, the conclusion~\eqref{eqn:liminfD10} in Lemma \ref{lem:nececondition} suggests that $D_1(G,G_0)$ may vanish at a much slower rate than $V(P_G,P_{G_0})$, i.e., the convergence of parameters representing $G$  may be much slower than the convergence of data distribution $P_G$. Moreover, the impact may be different for different types of parameters, as already noted in~\cite{ho2019singularity}. To explicate the distinct behavior for the mixing probability parameters $p_i$ and for the atoms $\theta_i$, define the following notion of distance,
for any $G=\sum_{i=1}^kp_i\delta_{\theta_i}\in \Ec_k(\Theta)$ and $G=\sum_{i=1}^kp'_i\delta_{\theta'_i}\in \Ec_k(\Theta)$, $r_1\geq 1$ and $r_2\geq 1$,
	\begin{equation}
	    \label{eqn:Dr1r2}
	D_{r_1,r_2}(G,G'):=\min_{\tau \in S_{k}} \sum_{i=1}^{k}\left(\|\theta_i-\theta'_{\tau(i)}\|_2^{r_1}+|p_i-p'_{\tau(i)}|^{r_2}\right).
	\end{equation}
Although $D_{r_1,r_2}$ might not be a proper metric, but by Lemma \ref{lem:relW1D1} \ref{item:relW1D1b} and similar to Lemma \ref{lem:relW1D1} \ref{item:relW1D1e},
for a fixed $G_0\in \Ec_k(\Theta)$, $D_{r,1}(G_0,G) \asymp_{G_0,\text{diam}(\Theta)} W_r^r(G_0,G)$ provided that $\Theta$ is bounded, i.e. there exists $c_1(G_0,\text{diam}(\Theta))$ and $c_2(\text{diam}(\Theta))$ such that for any $G\in \Ec_k(\Theta)$  
$$
c_1(G_0,\text{diam}(\Theta)) D_{r,1}(G_0,G) \leq W_r^r(G_0,G) \leq c_2(\text{diam}(\Theta)) D_{r,1}(G_0,G) .
$$ 
The conclusion of Lemma~\ref{lem:nececondition} can be refined further by the following result.

\begin{lem} [Impacts on different parameters] \label{lem:VD1r1r2lowbou} %\YW{move to appendix}
    Suppose all conditions in Lemma \ref{lem:nececondition} are satisfied. 
    \begin{enumerate}[label=\alph*)]
    \item \label{item:VD1r1r2lowboua}
    If at least one of $b_i$ is not zero, then for any $r\geq 1$
    $$
    \liminf_{\substack{G\overset{W_1}{\to} G_0\\ G\in \Ec_{k_0}(\Theta)}} \frac{V(P_G,P_{G_0})}{D_{r,1}(G,G_0)} =
    \liminf_{\substack{G\overset{W_1}{\to} G_0\\ G\in \Ec_{k_0}(\Theta)}} \frac{V(P_G,P_{G_0})}{W_{r}^{r}(G,G_0)}=0.
    $$

    \item \label{item:VD1r1r2lowboub}
    If at least one of $a_i$ is not zero, then for any $r\geq 1$
    $$
    \liminf_{\substack{G\overset{W_1}{\to} G_0\\ G\in \Ec_{k_0}(\Theta)}} \frac{V(P_G,P_{G_0})}{D_{1,r}(G,G_0)}=0.
    $$ 
    \end{enumerate}
\end{lem}

\begin{proof}[Proof of Lemma~\ref{lem:VD1r1r2lowbou}] 
The proof of \ref{item:VD1r1r2lowboub} is similar to that of \ref{item:VD1r1r2lowboua} and hence only the latter is presented. Let $G_\ell$ be the same as in the proof of Lemma \ref{lem:nececondition}. Then when $\ell$ is large $$
    D_{r,1}(G_\ell,G_0)=\sum_{i=1}^{k_0}\left(\|a'_i\|_2^{r}(1/\ell)^{r}+|b'_i|(1/\ell)\right) \geq 1/\ell\sum_{i=1}^{k_0}|b'_i| 
    $$
    and thus
    $$
    \frac{D_1(G_\ell,G_0)}{D_{r,1}(G_\ell,G_0)}\leq \frac{1/\ell}{1/\ell\sum_{i=1}^{k_0}|b'_i|}=\frac{1}{\sum_{i=1}^{k_0}|b'_i|}<\infty.
    $$
    Moreover, as shown in the proof of Lemma \ref{lem:nececondition},
    $$
     \lim_{\ell\to \infty}\frac{V(p_{G_\ell},p_{G_0})}{D_1(G_\ell,G_0)}=0.
    $$
    Combining the last two displays establishes 
    $$
    \liminf_{\substack{G\overset{W_1}{\to} G_0\\ G\in \Ec_{k_0}(\Theta)}} \frac{V(P_G,P_{G_0})}{D_{r,1}(G,G_0)} =0.
    $$
    It can be verified that for large $\ell$
    $$
    W_{r}^{r}(G,G_0) \geq \frac{1}{8}\left(\min_{1\leq i<j\leq k} \|\theta_i^0-\theta_j^0\|_2\right) \sum_{i=1}^k {|p_i^\ell-p_i^0|} = \frac{1}{8}\left(\min_{1\leq i<j\leq k} \|\theta_i^0-\theta_j^0\|_2\right) \frac{1}{\ell} \sum_{i=1}^{k_0}|b'_i|.
    $$
    The rest of the proof is similar to above to establish  
    $$ \liminf_{\substack{G\overset{W_1}{\to} G_0\\ G\in \Ec_{k_0}(\Theta)}} \frac{V(P_G,P_{G_0})}{W_{r}^{r}(G,G_0)}=0 .$$
\end{proof}


\section{moment map is injective}
We first show that $\lambda(\theta)$ is injective. By \eqref{eqn:Tmeangaussian}, for any $j\in [2k-1]$:
\begin{multline}
\lambda^{(j)}(\theta)=\sum_{i=1}^k \pi_i \left(\mu_i^j + \sum_{\ell=1}^\ell \sigma^{\ell} \E Y^\ell \mu_i^{j-\ell} \right) = \sum_{i=1}^k \pi_i \left(\mu_i^j + \sum_{\substack{\ell=2\\ \ell \text{ even}}}^j \sigma^{\ell} (\ell-1)!! \mu_i^{j-\ell} \right)\\
=\sum_{i=1}^k \pi_i \mu_i^j + \sum_{\substack{\ell=2\\ \ell \text{ even}}}^j \sigma^{\ell} (\ell-1)!! \sum_{i=1}^k \pi_i \mu_i^{j-\ell}. \label{eqn:lambdatelescope}
\end{multline}
Thus $\lambda(\theta)=\lambda(\bar{\theta})$ if and only if 
\begin{equation}
\sum_{i=1}^k \pi_i \mu_i^j = \sum_{i=1}^k \bar{\pi}_i \bar{\mu}_i^j,  \quad \forall j\in [2k-1]\cup\{0\}, \label{eqn:injectivegaussian}
\end{equation}
where the equation for $j=0$ is due to $\sum_{i=1}^k\pi_i=\sum_{i=1}^k\bar{\pi}_i=1$. Suppose that $\tilde{k}=|\{\mu_i\}_{i=1}^k \cap \{\bar{\mu}_i\}_{i=1}^k|<k$, and let $\{\mu_i\}_{i=1}^k \cup \{\bar{\mu}_i\}_{i=1}^k=\{\tilde{\mu}_i\}_{i=1}^{2k-\tilde{k}}$ be the distinct elements. Then the preceding displays can be written as 
\begin{equation}
\sum_{i=1}^{\tilde{k}} a_i\tilde{\mu}_i^j =0, \quad \forall j\in [k]\cup \{0\}. \label{eqn:Vandermondegaussian}
\end{equation}
There exists some $\tilde{\mu}_i\not \in \{\mu_i\}_{i=1}^k \cap \{\bar{\mu}_i\}_{i=1}^k$ and its coefficient $a_i$ is either $\pi_\ell$ or $-\bar{\pi}_\ell$ for some $\ell\in [k]$. But the coefficients of the first $\tilde{k}$ equations ($j=0,1,\ldots,\tilde{k}-1$) of system of linear equations \eqref{eqn:Vandermondegaussian} form a Vandermonde matrix and thus all $a_i=0$ for $i\in [\tilde{k}]$. That means for some $\ell\in [k]$, $\pi_\ell=0$ or $\bar{\pi}_\ell=0$, which is a contradiction. Hence $\tilde{k}=k$ and consequently $\mu_i=\bar{\mu}_i$ for $i\in [k]$. Then system of equations \eqref{eqn:injectivegaussian} become
$$
\sum_{i=1}^k (\pi_i-\bar{\pi}_i)\mu_i^j =0, \quad \forall j\in [2k-1]\cup \{0\}.
$$
Since the coefficients of the first $k$ equations ($j=0,1,\ldots,k-1$) form a Vandermonde matrix, the unique solution is $\pi_i=\bar{\pi}_i$ for $i\in [k]$. In conclusion, $\theta=\bar{\theta}$, which establishes that $\lambda(\theta)$ is injective.


\subsection{Data are equal-length exchangeable sequences}
	\label{sec:equal-length}
	Given $\n$ independent sequences of exchangeable observations of equal length $\m$, $X_{[\m]}^i = (X_{i1},X_{i2},\cdots,X_{i\m}) \in \Xfrak^{\m}$ for $i\in[\n]$. Each sequence $X_{[\m]}^i$ is assumed to be a sample drawn from a mixture of $\m-$product distributions $P_{G,\m}$ for some "true" de Finetti mixing measure $G=G_0 \in \Ec_{k_0}(\Theta)$. %\YW{As discussed in the first 2 or 3 (to be updated after the introduction is finalized) paragraphs in the introductions, $G_0$ is the de Finetti mixing measure and we are interested in estimate $G_0$ given $G_0\in \Ec_{k_0}(\Theta)$.}
	The problem is to estimate $G_0$ given the $m$ independent exchangeable sequences.
%	\marginpar{Not in arXiv}
	A Bayesian statistician endows upon $(\Ec_{k_0}(\Theta), \Bc(\Ec_{k_0}(\Theta)))$ a prior distribution $\Pi$ and obtains the posterior distribution $\Pi(dG| X^1_{[\m]},\ldots, X^{\n}_{[\m]})$ by Bayes' rule, where $\Bc(\Ec_{k_0}(\Theta))$ is the Borel sigma algebra w.r.t. $D_1$ distance. In this section we study the asymptotic behavior of this posterior distribution as the amount of data $\n\times\m$ tend to infinity. Later in Section~\ref{sec:variable-sized} we extend the posterior contraction theory to the more realistic setting where the $\n$ sequences are of variable lengths.
	
	 Suppose throughout this section,  $\{P_{\theta}\}_{\theta\in \Theta}$ has density $\{f(x|\theta)\}_{\theta\in \Theta}$ w.r.t. a $\sigma$-finite dominating measure $\mu$ on $\Xfrak$; %{\color{purple} can this be more general?}; \LN{possible, the main issue is to ensure assumption (B2) hold; also need to check Ghosal and vdV's theorems that were applied to} 
	 then $P_{G,\m}$ for $G=\sum_{i=1}^{k_0}p_i\delta_{\theta_i}$ has density w.r.t. to $\mu$:
	$$
	p_{G,\m}(\bar{x}) = \sum_{i=1}^{k_0} p_i\prod_{j=1}^{\m} f(x_j|\theta_i), \quad \text{for } \bar{x}=(x_1,x_2,\cdots,x_\m)\in \Xfrak^{\m}.
	$$
	Then the density of $X_{[\m]}^i$ conditioned on $G$ is $p_{G,\m}(\cdot)$.
	%
	Since $\Theta$ as a subset of $\R^q$ is separable, $\Ec_{k_0}(\Theta)$ is separable. Moreover, suppose the map $\theta\mapsto \P_\theta$ from $(\Theta,\|
	\cdot\|_2)$ to $(\{\P_\theta\}_{\theta\in \Theta}, h(\cdot,\cdot))$ is  continuous, where $h(\cdot,\cdot)$ is the Hellinger distance. Then the map from $ (\Ec_{k_0}(\Theta),D_1) \to (p_{G,\m},h(\cdot,\cdot))$ is also continuous by Lemma \ref{lem:hellingeruppbou}. Then by \cite[Lemma 4.51]{guide2006infinite}, $(x,G)\mapsto p_{G,\m}(x)$ is measurable for each $\m$. %{\color{purple} check this for general $\Xfrak$}
	Thus, the posterior distribution (a version of regular conditional distribution) is the random measure given by 
	$$
	\Pi(B|X_{[\m]}^1,X_{[\m]}^2,\ldots,X_{[\m]}^{\n}) = \frac{\int_B\prod_{i=1}^\n p_{G,\m}(X_{[\m]}^i)d\Pi(G)}{\int_{\Ec_{k_0}(\Theta)}\prod_{i=1}^\n p_{G,\m}(X_{[\m]}^i)d\Pi(G)} 
	$$ 
	for any Borel measurable subset of $B \subset \Ec_{k_0}(\Theta)$.	
	For further details of why the last quantity is a valid posterior distribution, we refer to Section 1.3 in \cite{ghosal2017fundamentals}. 
	%
	It is customary to express the above model equivalently in the hierarchical Bayesian fashion: 
	\begin{align*}
	&G \sim \Pi,  \quad \theta_1,\theta_2,\cdots,\theta_\n|G \overset{i.i.d.}{\sim} G\\
	&X_{i1},X_{i2},\cdots,X_{i\m} |\theta_i  \overset{i.i.d.}{\sim} f(x|\theta_i) \quad \text{for }i=1,\cdots,\n.
	\end{align*}
	As above, the $\n$ independent data sequences are denoted by $X_{[\m]}^i = (X_{i1},\cdots,X_{i\m}) \in \Xfrak^{\m }$ for $i\in[\n]$.
	

	 %\YW{A $k$-probability simplex is the set $\{x\in \R^s: \sum_{i=1}^k x_i =1 \text{ and } x_i\geq 0, \forall i\in [k]  \}.$} 
	 The following assumptions are required for the main theorems of this section.
	
	\begin{enumerate}[label=(B\arabic*)]
	
	\item \label{item:prior} (Prior assumption)  There is a prior measure $\Pi_{\theta}$ on $\Theta_1\subset \Theta$ with its Borel sigma algebra possessing a density w.r.t. Lebesgue measure that is bounded away from zero and infinity, where $\Theta_1$ is a compact subset of $\Theta$. Define $k_0$-probability simplex $\Delta^{k_0}:=\{(p_1,\ldots,p_{k_0}) \in \R_+^{k_0} | 
	\sum_{i=1}^{k_0} = 1\}$, Suppose there is a prior measure $\Pi_p$ on the $k_0$-probability simplex possessing a density w.r.t. Lebesgue measure on $\R^{k_0-1}$ that is bounded away from zero and infinity. Then $\Pi_p\times \Pi_{\theta}^{k_0}$ is a measure on $\{((p_1,\theta_1),\ldots,(p_{k_0},\theta_{k_0}))|p_i\geq 0, \theta_i\in \Theta_1, \sum_{i=1}^{k_0}p_i=1\}$, which induces a probability measure on $\Ec_{k_0}(\Theta_1)$. % identified as the quotient space of preceding space by the equivalence relationship of permutation invariance.\footnote{Rigorously speaking, $\Ec_{k_0}(\Theta_1)$ is only a proper subspace of the quotient space since a point in the quotient space might have $\theta_i = \theta_j$. But the set of such points have probability zero under the induced measure.} 
	Here, the prior $\Pi$ is generated by via independent $\Pi_p$ and $\Pi_\theta$ and the support $\Theta_1$ of $\Pi_\theta$ is such that $G_0\in \Ec_{k_0}(\Theta_1)$. 
	
	
%	\item \label{item:identifiableattruth}  (Identifiability at truth)  \YW{$n_0(G_0,\Theta_1)<\infty$.} \marginpar{not in arXiv}
	%There exists $n_0\geq 1$ such that map $G \mapsto P_{G,n_0}$ is identifiable at $G_0$ on $\bigcup_{k=1}^{k_0}\Ec_{k}(\Theta_1))$, i.e. for any $G\in \bigcup_{k=1}^{k_0}\Ec_{k}(\Theta_1))\backslash \{G_0\}$, $P_{G,n_0} \not= P_{G_0,n_0}$. 
	 
	
	
	\item \label{item:kernel} (Kernel assumption) Suppose that for every $\theta_1,\theta_2\in \Theta_1$, $\theta_0\in \{\theta_i^0\}_{i=1}^{k_0}$ and some positive constants $\alpha_0,L_1, \beta_0, L_2$,
	 \begin{align*}
	 K(f(x|\theta_0),f(x|\theta_2))\leq &L_1\|\theta_0-\theta_2\|_2^{\alpha_0}, \\
	 h(f(x|\theta_1),f(x|\theta_2))\leq & L_2\|\theta_1-\theta_2\|_2^{\beta_0}.
	 \end{align*}
	\begin{comment}
	Suppose $K(f(x|\theta_1),f(x|\theta_2))\leq L_1\|\theta_1-\theta_2\|_2^{\alpha_0}$ 
	for some $\alpha_0>0$ and some $L_1>0$.
	Suppose $h(f(x|\theta_1),f(x|\theta_2))\leq L_2\|\theta_1-\theta_2\|_2^{\beta_0}$ 
	for some $\beta_0>0$ and some $L_2>0$. Here $\theta_1,\theta_2$ are any distinct elements in $\Theta_1$.
	\end{comment}
	\end{enumerate}
	
	\begin{rem} \label{rem:Lippowerbou}
	\ref{item:prior} on the compactness of the support $\Theta_1$ is a standard assumption so as to obtain parameter convergence rate in finite mixture models (see~\cite{chen1995optimal,nguyen2013convergence,ho2016convergence,ho2016strong,ghosal2017fundamentals,heinrich2018strong, wu2020optimal}).
	See Section \ref{sec:compactness} for more discussions on the compactness assumption. In this paper, for simplicity we consider the prior on finite mixing measures being generated by independent priors on component parameters $\theta$ and an independent prior on mixing proportions $p_i$ \cite{Rousseau-Mengersen-11,nguyen2013convergence,guha2019posterior} for general probability kernel $\{f(x|\theta)\}$. It is not difficult to extend our theorem to more complex forms of prior specification when a specific kernel $\{f(x|\theta)\}$ is considered. 
	%\marginpar{not in arXiv}
    %\ref{item:prior} on the boundedness of the support $\Theta_1$ of prior distribution $\Pi_\theta$ is a standard assumption so as to obtain concrete rates of posterior contraction for the data population's distribution $P_G$ (cf.~\cite{ghosal2017fundamentals}). Moreover, the compactness of $\Theta_1$ is required in order to transfer the convergence rates of $P_G$ into that of $G$ (cf. Lemma~\ref{cor:VlowbouW1}). 
	

	The condition \ref{item:kernel} is not uncommon in parameter estimation (e.g. Theorem 8.25 in \cite{ghosal2017fundamentals}). Note that the conditions in \ref{item:kernel} imply some implicit constraints on $\alpha_0$ and $\beta_0$. Specifically,
	if \eqref{eqn:noproductlowbou} holds for $G_0\in \Ec_{k_0}(\Theta^\circ)$ and \ref{item:kernel} holds, then $\beta_0\leq 1$ and $\alpha_0\leq 2$. Indeed, for any sequence $G_\ell=\sum_{i=2}^{k_0} p^0_i\delta_{\theta_i^0} + p^0_1\delta_{\theta^\ell_1}\in\Ec_{k_0}(\Theta)\backslash \{G_0\}$ converges to $G_0=\sum_{i=1}^{k_0}p^0_i\delta_{\theta_i^0}$, by \eqref{eqn:noproductlowbou}, Lemma \ref{lem:Vupperbou} with $\m=1$ and \ref{item:kernel}, for large $\ell$
	\begin{multline} 
	C(G_0)\|\theta_1^\ell-\theta_1^0\|_2 = C(G_0)D_1(G_\ell,G_0) \leq V(P_{G_\ell},P_{G_0})\\ \leq V(f(x|\theta^\ell_1),f(x|\theta^0_1)) \leq h(f(x|\theta^\ell_1),f(x|\theta^0_1))\leq  L_2\|\theta_1^\ell-\theta^0_1\|^{\beta_0}_2,\label{eqn:hbeta0bou}
	\end{multline}
	which implies $\beta_0\leq 1$ (by dividing both sides by $\|\theta_1^\ell-\theta_1^0\|_2$ and letting  $\ell\to\infty$). In the preceding display $C(G_0)=\frac{1}{2}\liminf_{\substack{G\overset{W_1}{\to} G_0\\ G\in \Ec_{k_0}(\Theta)}} \frac{V(p_G,p_{G_0})}{D_1(G,G_0)}>0$.
	By \eqref{eqn:hbeta0bou} and Pinsker's inequality, 
	$$
	C(G_0)\|\theta_1^\ell-\theta_1^0\|_2\leq V(f(x|\theta^\ell_1),f(x|\theta^0_1))\leq \sqrt{\frac{1}{2}K(f(x|\theta^0_1),f(x|\theta^\ell_1))} \leq \sqrt{\frac{1}{2}L_1 \|\theta_1^\ell-\theta^0_1\|^{\alpha_0}_2},
	$$ for large $\ell$,
	which implies $\alpha_0\leq 2$. % if divide both sides by $\|\theta_1^\ell-\theta_1^0\|_2$ and let  $\ell\to\infty$. 
	The same conclusion holds if one replaces \eqref{eqn:noproductlowbou} with \eqref{eqn:genthmcon} by
	an analogous argument. 
	\myeoe
	\end{rem}



	\begin{thm} \label{thm:posconiid}	%\marginpar{not in arXiv}
		Fix $G_0\in\Ec_{k_0}(\Theta^\circ)$. Suppose  \ref{item:prior}, %\ref{item:identifiableattruth}, 
		\ref{item:kernel} and additionally \eqref{eqn:genthmcon} hold. 
		 %Let $n_1(G_0)$ be given by~\eqref{eqn:defn0n1n2}. \YW{Is this necessary? It also looks like the equation number (19) is only for the last equation.}
    \begin{enumerate}[label=\alph*)]
        \item \label{item:posconiida} 
        %[(i)] 
        There exists a constant $C(G_0)>0$ such that as $\n \rightarrow \infty$ while fixing $\m \geq n_1(G_0)\vee n_0(G_0,\cup_{k\leq k_0}\Ec_k(\Theta_1))$, for every $\bar{M}_\n\to \infty$, there holds
	$$
	\Pi \biggr (G\in \Ec_{k_0}(\Theta_1): D_{\m}(G,G_0) \geq C(G_0) \bar{M}_\n \sqrt{\frac{\ln(\n\m)}{\n}} \biggr  |X_{[\m]}^1,X_{[\m]}^2,\ldots,X_{[\m]}^{\n} \biggr ) \to 0
	$$
	in $\bigotimes^m \P_{G_0,N}$-probability as $\n\to \infty$.
	   \item \label{item:posconiidb} 
	   %[(ii)] 
	   If in addition, \eqref{eqn:noproductlowbou} is satisfied. Then the claim in part \ref{item:posconiida} holds with $n_1(G_0) = 1$.
	   \end{enumerate}
	\end{thm}


\begin{rem} %Implicit in the theorem's statement is that $n_0(G_0,\cup_{k\leq k_0}\Ec_k(\Theta_1)) \vee n_1(G_0) <\infty$; otherwise the admissible $N$ would be undefined. \blue{delete? this sentence reads confusing to me at first glance since it seems to indicate we have an implicit assumption. See the end of this paragraph}
%    By definition of $n_0(G_0,\cup_{k\leq k_0}\Ec_k(\Theta_1))$ in \eqref{eqn:defn0n1n2}, $P_{G,N}$ uniquely identifies $G_0$ when $N\geq n_0(G_0,\cup_{k\leq k_0}\Ec_k(\Theta_1))$, which is a necessary condition since otherwise there is no way to recover $G_0$. 
As discussed in Remark \ref{rem:claytonresult}, \cite{vandermeulen2019operator} establishes that $ n_0(G_0,\cup_{k\leq k_0}\Ec_k(\Theta))\leq 2k_0 -1$ for any $G_0\in \Ec_{k_0}(\Theta)$. While the uniform upper bound $2k_0-1$ might not be tight, it does show  $n_0(G_0,\cup_{k\leq k_0}\Ec_k(\Theta_1))<\infty$. By Proposition~\ref{lem:n0nbar} \ref{item:n1Nbar}, $n_1(G_0) < \infty$ is a direct consequence of \eqref{eqn:genthmcon}. Hence $n_0(G_0,\cup_{k\leq k_0}\Ec_k(\Theta_1)) \vee n_1(G_0) <\infty$.
\myeoe
    
   % On the other hand, the $n_0(G_0,\cup_{k\leq k_0}\Ec_k(\Theta_1))\leq n_0(G_0,\cup_{k\leq k_0}\Ec_k(\Theta^\circ))$ when $\Theta_1\subset \Theta^\circ$. In this case, due to Proposition~\ref{lem:n0nbar}~\ref{item:n2n0new}, it can be implied that $n_0(G_0,\cup_{k\leq k_0}\Ec_k(\Theta_1))<\infty$  provided~\eqref{eqn:curvatureprodbound} is satisfied for every  $G_0\in \Ec_{2 k_0}(\Theta^\circ)$, which holds for all full rank exponential family specified in Corollary \ref{cor:expfamtheta}, or for more general family by checking Theorem \ref{thm:genthm} for every $G_0\in \Ec_{2 k_0}(\Theta^\circ)$. 
\end{rem}


\begin{rem}
 In the above theorem, note that the constant $C(G_0)$ also depends on $\Theta_1$, $k_0$, $q$, upper and lower bounds of the densities of $\Pi_\theta$, $\Pi_p$ and the density family $f(x|\theta)$ (including $\alpha_0$, $\beta_0$, $L_1$, $L_2$ etc). All such dependence are suppressed for the sake of a clean presentation; it is the dependence on $G_0$ and the \emph{independence} of $\n,\m$ that we want to emphasize. Further remarks of Theorem \ref{thm:posconiid} are available as in Remark \ref{rem:consequenceofposcon} with $\bar{N}_m$ replaced by $N$, where we establish posterior contraction in a more general setting. \myeoe
\end{rem}

 The conditions \ref{item:kernel} and \eqref{eqn:genthmcon} can be verified for full rank exponential families and hence we have the following corollary from Theorem \ref{thm:posconiid}. %YW: this is modified from the previous paragraph, commented out below.


\begin{cor}  \label{cor:posconexp} 
Consider a full rank exponential family for kernel $P_\theta$ specified as in Corollary \ref{cor:expfamtheta} and assume all the requirements there are met. Fix $G_0\in \Ec_{k_0}(\Theta^\circ)$. Suppose that $\ref{item:prior}$ holds with $\Theta_1\subset \Theta^\circ$. Then the conclusions \ref{item:posconexpa}, \ref{item:posconexpb} of Theorem \ref{thm:posconiid} hold.
\begin{comment}
\begin{enumerate}[label=\alph*)]
    \item \label{item:posconexpa} 
    %[(i)] 
        There exist a constant $C(G_0)>0$ such that as $\n \rightarrow \infty$ while fixing $\m \geq n_1(G_0)\vee n_0(G_0,\cup_{k\leq k_0}\Ec_k(\Theta_1))$, for every $\bar{M}_\n\to \infty$, there holds
	$$
	\Pi \biggr (G\in \Ec_{k_0}(\Theta_1): D_{\m}(G,G_0) \geq C(G_0) \bar{M}_\n \sqrt{\frac{\ln(\n\m)}{\n}} \biggr  |X_{[\m]}^1,X_{[\m]}^2,\ldots,X_{[\m]}^{\n} \biggr ) \to 0
	$$
	in $\bigotimes^m \P_{G_0,N}$-probability as $\n\to \infty$.
	   \item \label{item:posconexpb} 
	   %[(ii)] 
	   If in addition, \eqref{eqn:noproductlowbou} is satisfied. Then the claim in part \ref{item:posconiida} holds with $n_1(G_0) = 1$.
	   \end{enumerate}
	   \end{comment}
\end{cor}


%\blue{I think the Corollary on exponential family is useful. It contains a large set of kernels and has simpler conditions since the inverse bound assumption and \ref{item:kernel} are already verified. to be discussed}
\begin{comment}
\LN{Recommend the following para and Cor 6.4 be removed}

\YW{ The condition \ref{item:kernel} can be verified for full rank exponential families and hence we have the following corollary from Theorem \ref{thm:posconiid}. YW: this is modified from the previous paragraph, commented out below.} \marginpar{not in arXiv}



%As already discussed in the Remark \ref{rem:Lippowerbou}, the condition \ref{item:identifiableattruth} is satisfied for full rank exponential families of kernels.  Indeed \ref{item:kernel} can also be verified for full rank exponential families and hence we have the following corollary from Theorem \ref{thm:posconiid}.

\begin{cor}  \label{cor:posconexp} \marginpar{not in arXiv}
Consider a full rank exponential family for kernel $P_\theta$ specified as in Corollary \ref{cor:expfamtheta} and assume all the requirements there are met.
Fix $G_0\in \Ec_{k_0}(\Theta^\circ)$. Suppose that $\ref{item:prior}$ holds with $\Theta_1\subset \Theta^\circ$. \begin{enumerate}[label=\alph*)]
    \item \label{item:posconexpa} 
    %[(i)] 
        There exist a constant $C(G_0)>0$ such that as $\n \rightarrow \infty$ while fixing \YW{$\m \geq n_1(G_0)\vee n_0(G_0,\cup_{k\leq k_0}\Ec_k(\Theta_1))$}, for every $\bar{M}_\n\to \infty$, there holds
	$$
	\Pi \biggr (G\in \Ec_{k_0}(\Theta_1): D_{\m}(G,G_0) \geq C(G_0) \bar{M}_\n \sqrt{\frac{\ln(\n\m)}{\n}} \biggr  |X_{[\m]}^1,X_{[\m]}^2,\ldots,X_{[\m]}^{\n} \biggr ) \to 0
	$$
	in $\bigotimes^m \P_{G_0,N}$-probability as $\n\to \infty$.
	   \item \label{item:posconexpb} 
	   %[(ii)] 
	   If in addition, \eqref{eqn:noproductlowbou} is satisfied. Then the claim in part \ref{item:posconiida} holds with $n_1(G_0) = 1$.
	   \end{enumerate}
\end{cor}

\end{comment}
%Let us apply Corollary \ref{cor:posconexp} to the Bernoulli kernel and two-paramters Gamma kernel.

\begin{exa}[Posterior contraction for weakly identifiable kernels: Bernoulli and gamma] %\marginpar{not in arXiv}

Fix $G_0\in \Ec_{k_0}(\Theta^\circ)$.  
%
For the Bernoulli kernel studied in Example \ref{exa:bernoulli}, $n_1(G_0)=n_0(G_0,\cup_{k\leq k_0}\Ec_k(\Theta))=2k_0-1$. Suppose that $\ref{item:prior}$ holds with compact $\Theta_1\subset \Theta^\circ=(0,1)$. 
%Then the conclusion \ref{item:posconexpa} in Corollary \ref{cor:posconexp} holds for any $N\geq 2k_0-1$. 
It is easily verified that the conclusion of Thm~\ref{thm:posconiid} holds for any $N\geq 2k_0-1$.
%
For the gamma kernel studied in Example \ref{exa:gamma}, \ref{exa:gamma2}, $n_1(G_0) = 2$ when $G_0\in \Gc$ and $n_1(G_0)=1$ when $G_0\in \Ec_{k_0}(\Theta^\circ)\backslash \Gc$; $n_0(G_0,\cup_{k\leq k_0}\Ec_k(\Theta))=1$. Suppose that $\ref{item:prior}$ holds with compact $\Theta_1\subset \Theta^\circ=(0,\infty)\times (0,\infty)$. 
%Then the conclusion \ref{item:posconexpa} in Corollary \ref{cor:posconexp} 
The conclusion of Theorem~\ref{thm:posconiid}
holds for any $N\geq 2$. Moreover, the same conclusion holds for $N\geq 1$ if $G_0\not \in \Gc$ is given. \myeoe
\end{exa}


\begin{comment}
\begin{exa}[Posterior contraction for Examples \ref{exa:uniformcontinue}, \ref{exa:exponentialcontinuerevision}, \ref{exa:kernelmixture} and \ref{exa:dirichlet}] \marginpar{not in arXiv}

Fix $G_0\in \Ec_{k_0}(\Theta^\circ)$.  
%
 Suppose that $\ref{item:prior}$ holds with \YW{compact $\Theta_1\subset \Theta^\circ$}. Then the conclusion \ref{item:posconexpa} in Corollary \ref{cor:posconexp} holds for any $N\geq 2k_0-1$. 
%
For the gamma kernel studied in Example \ref{exa:gamma}, \ref{exa:gamma2}, $n_1(G_0) = 2$ when $G_0\in \Gc$ and $n_1(G_0)=1$ when $G_0\in \Ec_{k_0}(\Theta^\circ)\backslash \Gc$; \YW{$n_0(G_0,\Theta)=1$}. Suppose that $\ref{item:prior}$ holds with \YW{compact $\Theta_1\subset \Theta^\circ=(0,\infty)\times (0,\infty)$}. Then the conclusion \ref{item:posconexpa} in Corollary \ref{cor:posconexp} holds for any $N\geq 2$. Moreover, the same conclusion holds with $N\geq 1$ if additional information $G_0\not \in \Gc$ is known. \myeoe
\end{exa}
\end{comment}


	\subsection{Data are variable-length exchangeable sequences}
	\label{sec:variable-sized}
Now we turn to a realistic setting where the $\n$ observed exchangeable sequences are of variable lengths.  For $i=1,2,\cdots, \n$, 
	denote $X_{[\m_i]}^i = (X_{i1},X_{i2},\cdots,X_{i\m_i}) \in \Xfrak^{\m_i }$, where $\m_i$ is the length of $X^i_{[\m_i]}$ sequence. Consider the hierarchical model:
	\begin{align*}
	&G \sim \Pi,  \quad \theta_1,\theta_2,\cdots,\theta_\n|G \overset{i.i.d.}{\sim} G\\
	&X_{i1},X_{i2},\cdots,X_{i\m_i} |\theta_i  \overset{i.i.d.}{\sim} f(x|\theta_i) \quad \text{for }i=1,\cdots,\n.
	\end{align*}

	
As in Section~\ref{sec:equal-length}, the probability family $\{P_{\theta}\}_{\theta\in \Theta}$ has density $\{f(x|\theta)\}_{\theta\in \Theta}$ w.r.t. a $\sigma$-finite measure $\mu$ on $\Xfrak$; then $P_{G,\m_i}$ for $G=\sum_{i=1}^{k_0}p_i\delta_{\theta_i}$ has density w.r.t. to $\mu$:
	\begin{equation}
	p_{G,\m_i}(\bar{x}) = \sum_{i=1}^{k_0} p_i\prod_{j=1}^{\m_i} f(x_j|\theta_i), \quad \text{for } \bar{x}=(x_1,x_2,\cdots,x_{\m_i})\in \Xfrak^{\m_i}.  \label{eqn:pGNdef}
   \end{equation}
	Then the density of $X_{[\m_i]}^i$ conditioned on $G$ is $p_{G,\m_i}(\cdot)$.
	Thus, given the $\n$ data sequences $X^1_{[\m_1]},\ldots, X_{[\m_\n]}^{\n}$, the posterior distribution of mixing measure $G$ is given by 
	$$
	\Pi(B|X_{[\m_1]}^1,\ldots,X_{[\m_{\n}]}^{\n}) = \frac{\int_B\prod_{i=1}^\n p_{G,\m_i}(X_{[\m_i]}^i)d\Pi(G)}{\int_{\Ec_{k_0}(\Theta)}\prod_{i=1}^\n p_{G,\m_i}(X_{[\m_i]}^i)d\Pi(G)} \;\text{for any measurable}\, B \subset \Ec_{k_0}(\Theta).
	$$
	

	An useful quantity is the average sequence length
	$$\bar{\m}_{\n}=\frac{1}{\n}\sum_{i=1}^{\n}\m_i.
	$$
	The posterior contraction theorem will be characterized in terms of distance $D_{\bar{\m}_{\n}}(\cdot, \cdot)$, which extends the original notion of distance $D_\m(\cdot,\cdot)$ by allowing real-valued weight $\bar{\m}_{\n}$. %Specifically, for any real $r>0$,  for $G=\sum_{i=1}^{k_0}p_i\delta_{\theta_i}\in \Ec_{k_0}(\Theta)$ and $G'=\sum_{i=1}^{k_0}p'_i\delta_{\theta'_i}\in \Ec_{k_0}(\Theta)$ define
	%\[\myD_{r}(G,G') =  \min_{\tau\in S_{k_0}} \sum_{i=1}^{k_0}(\sqrt{r}\|\theta_{\tau(i)}-\theta'_i\|_2+|p_{\tau(i)}-p'_i|),\] 
	%where $S_{k_0}$ denotes the set of all permutations on the set $[k_0]$. 
	

	\begin{thm}\label{thm:posconnotid} 
	Fix $G_0\in\Ec_{k_0}(\Theta^\circ)$. Suppose  \ref{item:prior}, %\ref{item:identifiableattruth}, 
		\ref{item:kernel} and additionally \eqref{eqn:genthmcon} hold. 
	\begin{enumerate}[label=\alph*)]
	  \item \label{item:posconnotida} 
	  There exists some constant $C(G_0)>0$ such that as long as $n_0(G_0,\cup_{k\leq k_0}\Ec_k(\Theta_1)) \vee n_1(G_0) \leq \min_{i} \m_i \leq \sup_{i} \m_i < \infty$, for every $\bar{M}_\n\to \infty$ there holds
	\begin{align*}
	&\Pi \biggr (G\in \Ec_{k_0}(\Theta_1): D_{\bar{\m}_{\n}}(G,G_0) \geq C(G_0)\bar{M}_\n \sqrt{ \frac{\ln(\n\bar{\m}_{\n})}{\n} } \biggr |X_{[\m_1]}^1, \ldots,X_{[\m_{\n}]}^{\n} \biggr ) \to  0
	\end{align*}
	in $\bigotimes_{i=1}^{m}\P_{G_0,\m_i}$-probability as $\n\to \infty$.
	
	\item \label{item:posconnotidb}
	If in addition, ~\eqref{eqn:noproductlowbou} is satisfied. Then the claim in part \ref{item:posconnotida} holds with $n_1(G_0) = 1$.
	\end{enumerate}
	\end{thm}
	
%	We make the following remarks.
	\begin{rem} \label{rem:consequenceofposcon}
	\label{rem:posconnotiid}
%	\begin{enumerate}[label=\alph*)]
%	 \item %[(a)] 
	 (a) In the above statement, note that the constant $C(G_0)$ also depends on $\Theta_1$, $k_0$, $q$, upper and lower bounds of the densities of $\Pi_\theta$, $\Pi_p$ and the density family $f(x|\theta)$ (including $\alpha_0$, $\beta_0$, $L_1$, $L_2$ etc). All such dependence are suppressed for the sake of a clean presentation; it is the dependence on $G_0$ and the \emph{independence} of $\n,\{\m_i\}_{i\geq 1}$ and $\m_0:=\sup_{i}\m_i < \infty$, that we want to emphasize. In addition, although $C(G_0)$ and hence the vanishing radius of the ball characterized by $D_{\bar{\m}_\n}$ does \emph{not} depend on $\m_0$, the rate at which the posterior probability statement concerning this ball tending to zero may depend on it.
	
%	\item %[(b)] 
	(b) Roughly speaking, the theorem produces the following posterior contraction rates. The rate toward mixing probabilities $p_i^0$ is $O_P((\ln(\n\bar{\m}_\n)/\n)^{1/2})$. 
   Individual atoms $\theta_i^0$ have much faster contraction rate, which utilizes the full volume of the data set: 
   \begin{equation}
   O_P\left(\sqrt{\frac{\ln(\n\bar{\m}_\n)}{\n\bar{\m}_\n}}\right) = 
   O_P\biggr (\sqrt{\frac{\ln (\sum_{i=1}^{\n} \m_i)}{\sum_{i=1}^{\n} \m_i}} \biggr). \label{eqn:atomconvergencerate}
   \end{equation}
	Note that the condition that $\sup_i N_i<\infty$ implies that $\bar{N}_m$ remains finite when $m\to \infty$. Since constant $C(G_0)$ is independent of $\bar{N}_m$ and $m$, the theorem establishes that the larger the average length of observed sequences, the faster the posterior contraction as $m\to \infty$. \blue{The current sentence seems a little vague and do not 
	Is my previous sentence more informative? ``The whole picture is that increasing $N_i$ from $1$ to $n_1(G_0)\vee n_0(G_0,\cup_{k\leq k_0}\Ec_k(\Theta_1))$ will guarantee a rate $m^{-1/2}$ (moderate some $\log$ factor) and overcome the slow convergence rate for the weak identifiable family, like mixture of Gamma in Example \ref{exa:gamma}. Once beyond the threshold $n_1(G_0)\vee n_0(G_0,\cup_{k\leq k_0}\Ec_k(\Theta_1))$, increasing $N_i$ will continue to reduce the constant coefficient of the rate $m^{-1/2}$.''  Related to R2 comment \# 6} 
	%\marginpar{not in arXiv}
	
%	\item %[(c)]
	(c) The distinction between the two parts of the theorem highlights the role of first-order identifiability in mixtures of $\m$-product distributions. Under first-order identifiability, ~\eqref{eqn:noproductlowbou} is satisfied, so we can establish the aforementioned posterior contraction behavior for a full range of sequence length $\m_i$'s, as long as they are uniformly bounded by an arbitrary unknown constant. When first-order identifiability is not satisfied, so~\eqref{eqn:noproductlowbou} may fail to hold, the same posterior behavior can be ascertained when the sequence lengths exceed certain threshold depending on the true $G_0$, namely, $n_1(G_0)\vee n_0(G_0,\cup_{k\leq k_0}\Ec_k(\Theta_1))$.
	
	(d) The proof of Theorems~\ref{thm:posconiid} and~\ref{thm:posconnotid}  utilizes general techniques of Bayesian asymptotics (see  \cite[Chapter 8]{ghosal2017fundamentals}) to deduce posterior contraction rate on the   density $h(P_{G,N},P_{G_0,N})$. The main novelty lies in the 
	 application of 
	 inverse bounds for mixtures of product distributions of exchangeable sequences established in Section~\ref{sec:inversebounds}. These are lower bounds of distances  $h(P_{G_0,\m},P_{G,\m})$ between a pair of distributions ($P_{G_0,\m}, P_{G,\m}$) in terms of distance $D_{\m}(G_0,G)$  between the corresponding $(G_0,G)$. The distance $D_{\m}(G_0,G)$ brings out the role of the sample size $\m$ of exchangeable sequences, resulting in the rate $\m^{-1/2}$ (or $\bar{N}_m^{-1/2}$, modulo the logarithm). % Under suitable identifiability and regularity conditions we established the convergence of certain mixing parameters with a rate proportional to $\m^{-1/2}$. 
	 %In Appendix \ref{sec:minimax}, we shall prove the sharpness of the inverse bounds obtained, by presenting suitable opposing upper bounds. These upper bounds are also useful in establishing minimax theorems for the estimation of mixing measures.  \blue{the last sentence is not true since the minimax rate only uses Lemma \ref{lem:hellingeruppbou} but not Lemma \ref{lem:optimalsquaretootN}. Also is a sentence on minimax important? Remove it?}
	 %\YW{Looks like this is new. Do you also want to add this to the axkiv version?}
	%\YW{the question mark to be corrected}
%	\end{enumerate} 
\myeoe
	\end{rem}
	
%	\section{Sharpness of bounds and minimax theorem}
%	\label{sec:minimax}


\section{Proof of equal length}	
\begin{proof}[Proof of Theorem \ref{thm:posconiid}] 



%\begin{enumerate}[label=\alph*)]
a) %\item 
We verify conditions (i) and (ii) of  \cite[Theorem 8.11]{ghosal2017fundamentals} respectively in Step 1 and Step 2 below to obtain a posterior contraction on the density estimation. In Step 3 we apply Lemma \ref{cor:identifiabilityallm} to transfer the posterior contraction result on density estimation to parameter estimation. We begin with the following two useful inequalities relating Hellinger distance to $W_1$ and $D_N$.

Write $n_1$ and $n_0$ respectively for $n_1(G_0)$ and $n_0(G_0,\cup_{k\leq k_0} \Ec_k(\Theta_1))$ in the proof for clean presentation. 
Note that \ref{item:kernel} implies that $\theta\mapsto P_\theta$ from $(\Theta,\|\cdot\|_2)$ to $(\{P_\theta\}_{\theta\in \Theta}, h)$ is continuous. Then due to Lemma \ref{cor:VlowbouW1} and Lemma \ref{lem:relW1D1} \ref{item:relW1D1e}, for any $\m \geq n_1\vee n_0$,
	\begin{multline}
	\label{eqn:lowboundhwd}
	h(p_{G,\m},p_{G_0,\m}) \geq V(p_{G,\m},p_{G_0,\m})
	\geq C(G_0,\Theta_1)W_1(G,G_0)\\
	\geq  C(G_0,\Theta_1)D_1(G,G_0), \quad \forall G\in\Ec_{k_0}(\Theta_1). 
	\end{multline}
	Moreover, by Lemma \ref{cor:identifiabilityallm} for any $\m\geq n_1$ and for any $ G\in\Ec_{k_0}(\Theta_1): W_1(G,G_0)<c(G_0,\m)$
    \begin{equation}
    h(p_{G,\m},p_{G_0,\m})\geq V(p_{G,\m},p_{G_0,\m})\geq C(G_0)D_{\m}(G,G_0) \quad  \label{eqn:VnDnlowboulargen}
    \end{equation}
    where $c(G_0,\m)$ is a constant that depends on $G_0$ and $\m$. In the remainder of the proof $\m\geq n_1\vee n_0$ is implicitly imposed. \\
    
\noindent {\bf Step 1}(Verification of condition (i) of \cite[Theorem 8.11]{ghosal2017fundamentals}) \\
     By \eqref{eqn:lowboundhwd}, for any $\epsilon > 0$,
	\begin{equation}
	\{G\in \Ec_{k_0}(\Theta_1): h(p_{G,\m},p_{G_0,\m}) \leq \epsilon \} \subset \left\{G\in \Ec_{k_0}(\Theta_1): D_1(G,G_0)\leq \frac{\epsilon}{C(G_0,\Theta_1)}\right\}. \label{eqn:setinclusionhD1}
	\end{equation}
	Recall that $\Theta_1\subset \Theta \subset \R^q$ and $\Pi$ is supported on $\Ec_{k_0}(\Theta_1)$. Then for any $j \in \mathbb{N}$, by \eqref{eqn:setinclusionhD1}
	\begin{align}
	\Pi\left(h(p_{G,\m},p_{G_0,\m}) \leq 2j\epsilon\right) \leq \Pi\left(D_1(G,G_0)\leq \frac{2j\epsilon}{C(G_0,\Theta_1)}\right) \nonumber \\
	\lesssim %{\color{red} notation introduce} 
	k_0! \left( \frac{2j\epsilon}{C(G_0,\Theta_1)}\right)^{k_0-1} \left( \frac{2j\epsilon}{C(G_0,\Theta_1)}\right)^{qk_0}, \label{eqn:pih}
	\end{align}
	where the last inequality follows from \ref{item:prior}.
	
	Using the argument similar to \cite[Lemma 3.2 (a)]{nguyen2016borrowing} %{\color{purple} should we prove this since there your result involve dirichlet process.}, 
	for any $G=\sum_{i=1}^{k_0}p_i\delta_{\theta_i}\in \Ec_{k_0}(\Theta_1)$
	\begin{align*}
	K(p_{G_0,\m}, p_{G,\m}) \leq & \m L_1 W_{\alpha_0}^{\alpha_0}(G,G_0)\\ \leq & C(\text{diam}(\Theta_1),\alpha_0,L_1) \m  \min_{\tau\in S_{k_0}} \sum_{i=1}^{k_0}\left(\|\theta_{\tau(i)}-\theta^0_{i}\|_2^{\alpha_0} + |p_{\tau(i)}-p^0_i|  \right),
	\end{align*}
	where the first inequality follows from \ref{item:kernel} and the second inequality follows from Lemma \ref{lem:relW1D1} \ref{item:relW1D1b}. Then 
	\begin{equation}
	\Pi\left(K(p_{G_0,\m},p_{G,\m}) \leq \epsilon^2     \right)  \gtrsim \left( \frac{\epsilon^2}{ C(\text{diam}(\Theta_1),\alpha_0, L_1)\m}\right)^{qk_0/\alpha_0} \left( \frac{\epsilon^2}{ C(\text{diam}(\Theta_1),\alpha_0, L_1)\m}\right)^{k_0-1}. \label{eqn:piKlow}
	\end{equation}
	
	Combining \eqref{eqn:pih} and \eqref{eqn:piKlow},
	\begin{multline*}
	\frac{\Pi\left(h(p_{G,\m},p_{G_0,\m}) \leq 2j\epsilon\right)}{\Pi\left( K(P_{G_0,\m},P_{G,\m}) \leq \epsilon^2     \right)} \\
	\leq C(G_0,\Theta_1,q,\alpha_0,k_0, L_1) j^{qk_0+k_0-1} \m^{qk_0/\alpha_0+k_0-1}\epsilon^{-qk_0(2/\alpha_0-1)-(k_0-1)}.
	\end{multline*}
	By Remark \ref{rem:Lippowerbou} $\alpha_0 \leq 2$.
	Then based on the last display one may verify with \[\epsilon_{\n,\m}=C(G_0,\Theta_1,q,k_0,\alpha_0,\beta_0,L_1, L_2) \sqrt{\frac{\ln(\n\m)}{\n}}\] 
	for some large enough constant $C(G_0,\Theta_1,q,k_0,\alpha_0,\beta_0)$,
	$$ 
	\frac{\Pi\left(h(p_{G,\m},p_{G_0,\m}) \leq 2j\epsilon_{\n,\m}\right)}{\Pi\left( K(p_{G_0,\m},p_{G,\m}) \leq \epsilon^2_{\n,\m} \right)  } \leq \exp\left(\frac{1}{8}j\n\epsilon_{\n,\m}^2\right).
	$$
	\\
	
\noindent {\bf Step 2}(Verification of condition (ii) of Theorem 8.11 in \cite{ghosal2017fundamentals})\\
By \eqref{eqn:setinclusionhD1},
	\begin{align*}
	&\sup_{\epsilon\geq \epsilon_{\n,\m}} \ln \Nf\left(\frac{1}{2}\epsilon,\{p_{G,\m}: G\in \Ec_{k_0}(\Theta_1), h(p_{G,\m},p_{G_0,\m})\leq 2\epsilon \}, h\right)\\ 
	\leq & 
	\sup_{\epsilon\geq \epsilon_{\n,\m}} \ln \Nf\left(\frac{1}{2}\epsilon,\left\{p_{G,\m}: G\in \Ec_{k_0}(\Theta_1), D_1(G,G_0)\leq \frac{2\epsilon}{C(G_0,\Theta_1)}\right \}, h \right) \\
	\leq &  qk_0\ln \left(1+\frac{4\times (8L_2)^{\frac{1}{\beta_0}}}{C(G_0,\Theta_1)}  \m^{\frac{1}{2\beta_0}}\epsilon_{\n,\m}^{-(\frac{1}{\beta_0}-1)} \right)+(k_0-1)\ln \left(1+160\epsilon_{\n,\m}^{-2}\right),
	\end{align*}
	where the last inequality follows from Lemma \ref{lem:Nuppbou}. By Remark \ref{rem:Lippowerbou} $\beta_0 \leq 1$. Then based on the last display one may verify with \[\epsilon_{\n,\m}=C(G_0,\Theta_1,q,k_0,\alpha_0,\beta_0, L_1, L_2) \sqrt{\frac{\ln(\n\m)}{\n}}\]
	for some large enough constant $C(G_0,\Theta_1,q,k_0,\alpha_0,\beta_0)$,
	$$
	\sup_{\epsilon\geq \epsilon_{\n,\m}}\ln \Nf\left(\frac{1}{2}\epsilon,\{p_{G,\m}: G\in \Ec_{k_0}(\Theta_1), h(p_{G,\m},p_{G_0,\m})\leq 2\epsilon \}, h\right) \leq \n\epsilon^2_{\n,\m}.
	$$
    Now we invoke \cite[Theorem 8.11]{ghosal2017fundamentals} (the Hellinger distance defined in \cite{ghosal2017fundamentals} differs from our definition by a factor of constant. But this constant factor only affects the coefficients of $\epsilon_{\n,\bar{\m}_{\n}}$, not the conclusion of convergence),
	%\footnote{The Hellinger distance defined in \cite{ghosal2017fundamentals} differs from our definition by a factor of constant. But this constant factor only affect the coefficients of $\epsilon_{\n,\bar{\m}_{\n}}$ but not the conclusion of convergence.}, 
	 for every $\bar{M}_\n\to \infty$,  
	\begin{equation}
	\Pi(G\in \Ec_{k_0}(\Theta_1): h(p_{G,\m},p_{G_0,\m}) \geq \bar{M}_\n \epsilon_{\n,\m} |X_{[\m]}^1,X_{[\m]}^2,\ldots,X_{[\m]}^{\n} ) \to 0  \label{eqn:vanposcontraction}
	\end{equation}
	in $\bigotimes^m \P_{G_0,N}$-probability as $\n\to\infty$ while fixing $\m$. \\
	
\noindent {\bf Step 3} (From convergence of densities to that of parameters) \\
	 By \eqref{eqn:VnDnlowboulargen} and applying the union bound,
	\begin{align*}
	&\Pi\left(G\in \Ec_{k_0}(\Theta_1): D_{\m}(G,G_0) \geq \frac{\bar{M}_\n}{C(G_0)} \epsilon_{\n,\m} |X_{[\m]}^1,X_{[\m]}^2,\ldots,X_{[\m]}^{\n} \right) \\
	\leq  &\Pi\left(G\in \Ec_{k_0}(\Theta_1): h(p_{G,\m},p_{G_0,\m}) \geq \bar{M}_\n \epsilon_{\n,\m} |X_{[\m]}^1,X_{[\m]}^2,\ldots,X_{[\m]}^{\n} \right) \\
	& \quad + \Pi(W_1(G,G_0)>c(G_0,\m) |X_{[\m]}^1,X_{[\m]}^2,\ldots,X_{[\m]}^{\n} )\\
	\to & 0
	\end{align*}
	in $\bigotimes^m \P_{G_0,N}$-probability as $\n\to\infty$ by applying \eqref{eqn:vanposcontraction} to the first term. The reason the second term vanishes is as follows. Note that the second term converging to $0$ essentially is a posterior consistency result with respect to $W_1$ metric. Here, we prove it by \eqref{eqn:lowboundhwd} and \eqref{eqn:vanposcontraction}. 
	%\marginpar{not in arXiv} 
	By \eqref{eqn:lowboundhwd}
	\begin{align*}
	&\{G\in \Ec_{k_0}(\Theta_1): W_1(G,G_0)>c(G_0,\m)\}\\ 
	\subset& \{G\in\Ec_{k_0}(\Theta_1): h(p_{G,\m},p_{G_0,\m})> C(G_0,\m,\Theta_1) \} 
	\end{align*}
	for some constant $C(G_0,\m,\Theta_1)$. 
	%\LN{what is this $\rho$?}{\color{purple} Done!} 
	For some slow-increasing $\bar{M}'_{\n}$ such that $\bar{M}'_{\n}\epsilon_{\n,\m}\to 0$ as $\n\to \infty$, 
	\begin{align*}
	&\{G\in\Ec_{k_0}(\Theta_1): h(p_{G,\m},p_{G_0,\m})> C(G_0,\m,\Theta_1) \} \\
	\subset &\{G\in\Ec_{k_0}(\Theta_1): h(p_{G,\m},p_{G_0,\m})>\bar{M}'_{\n}\epsilon_{\n,\m}\}
	\end{align*}
	holds for large $\n$. Combining the last two displays and \eqref{eqn:vanposcontraction} 
	yields as $\n\to \infty$ 
	$$
	\Pi(G\in\Ec_{k_0}(\Theta_1): W_1(G,G_0)>c(G_0,\m) |X_{[\m_1]}^1,\ldots,X_{[\m_{\n}]}^{\n} )\\
	\to  0.
	$$

b) %\item 
If the additional condition of part \ref{item:posconiidb} is satisfied, then by Remark~\ref{rem:N1Ninfcon}, $n_1(G_0)=1$. That is, the claim of part \ref{item:posconiida} holds for $n_1(G_0) = 1$. 

%, i.e., ~\eqref{eqn:noproductlowbou} holds. Then we may apply Lemma \ref{cor:VlowbouW1} \ref{item:VD1r1r2lowboub} and Lemma \ref{lem:relW1D1} \ref{item:relW1D1e} to obtain that \eqref{eqn:lowboundhwd} holds for any $\m\geq \underbar{\m}_1=1$. Applying Lemma \ref{cor:identifiabilityallm}  \ref{item:identifiabilityallma} with $\m_0=\m$ one obtains that \eqref{eqn:VnDnlowboulargen} holds for $\m\geq \underbar{\m}_2=1$. Then repeat the proof of part \ref{item:posconiida} after \eqref{eqn:VnDnlowboulargen} and then the conclusion is established under $\underbar{\m}=1$. 

%\end{enumerate}
\end{proof}
	
	
\begin{lem} \label{lem:Nuppbou}
	Fix $G_0\in\Ec_{k_0}(\Theta_1)$. Suppose $h(f(x|\theta_1),f(x|\theta_2))\leq L_2\|\theta_1-\theta_2\|_2^{\beta_0}$ 
	for some $0<\beta_0\leq 1$ and some $L_2>0$ where $\theta_1, \theta_2$ are any two distinct elements in $\Theta_1$.
	\begin{align*}
	& \Nf\left(\frac{1}{2}\epsilon,\left\{p_{G,\m}: G\in \Ec_{k_0}(\Theta_1), D_1(G,G_0)\leq \frac{2\epsilon}{C(G_0,\text{diam}(\Theta_1))}\right \}, h \right)\\
	\leq &
	\left(1+\frac{4\times (8L_2)^{\frac{1}{\beta_0}}}{C(G_0,\text{diam}(\Theta_1))}  \m^{\frac{1}{2\beta_0}}\epsilon^{-(\frac{1}{\beta_0}-1)} \right)^{qk_0} \left(1+160\epsilon^{-2}\right)^{k_0-1}.
	\end{align*}
\end{lem}

\begin{proof}[Proof of Lemma \ref{lem:Nuppbou}]
	Consider an $\eta_1$-net $\Lambda_i$ with minimum cardinality of $\{\theta: \|\theta-\theta^0_i\|_2 \leq \frac{2\epsilon}{C(G_0,\text{diam}(\Theta_1))} \}$ and an $\eta_2$-net $\bar{\Lambda}$ with minimum cardinality  of $k_0$-probability simplex $\{p\in \R^{k_0}: \sum_{i=1}^{k_0}p_i =1, p_i\geq 0  \}$ under the $l_1$ distance. Construct a set $\tilde{\Lambda}=\{\tilde{G}=\sum_{i=1}^{k_0}p_i\delta_{\theta_i}: (p_1,\ldots,p_{k_0})\in \bar{\Lambda}, \theta_i\in \Lambda_i  \}$. Then for any  $G\in \Ec_{k_0}(\Theta)$ satisfying $ D_1(G,G_0)\leq \frac{2\epsilon}{C(G_0,\text{diam}(\Theta_1))}$, there exists some $\tilde{G}\in \tilde{\Lambda}$, such that by Lemma \ref{lem:hellingeruppbou}
	$$
	h(p_{G,\m},p_{\tilde{G},\m}) \leq \sqrt{\m} L_2 \eta_1^{\beta_0} + \frac{1}{\sqrt{2}}\sqrt{\eta_2}.
	$$
	Thus $\left\{p_{G,\m}: G\in \tilde{\Lambda} \right\}$ is a $\left(\sqrt{\m} L_2 \eta_1^{\beta_0} + \frac{1}{\sqrt{2}}\sqrt{\eta_2}\right)$-net of 
	$$
	\left\{p_{G,\m}: G\in \Ec_{k_0}(\Theta_1), D_1(G,G_0)\leq \frac{2\epsilon}{C(G_0,\text{diam}(\Theta_1))}\right \}.
	$$ 
	Since $\tilde{\Lambda}$ is not necessarily subset of $\Ec_{k_0}(\Theta_1)$,
	\begin{align}
	\Nf\left(2\left(\sqrt{\m} L_2 \eta_1^{\beta_0} + \frac{1}{\sqrt{2}}\sqrt{\eta_2}\right),\left\{p_{G,\m}: G\in \Ec_{k_0}(\Theta_1), D_1(G,G_0)\leq \frac{2\epsilon}{C(G_0,\text{diam}(\Theta_1))}\right \}, h \right)\nonumber \\
	\leq |\tilde{\Lambda}| = |\bar{\Lambda}|\prod_{i=1}^{k_0}|\Lambda_i|. \label{eqn:Nuppbou1}
	\end{align}
	Now specify $\eta_1=\left(\frac{\epsilon}{8L_2\sqrt{\m}}\right)^{\frac{1}{\beta_0}}$ and thus 
	$$
	|\Lambda_i|\leq \left(1+2\frac{2\epsilon}{C(G_0,\text{diam}(\Theta_1))}/\eta_1\right)^q = \left(1+\frac{4\times (8L_2)^{\frac{1}{\beta_0}}}{C(G_0,\text{diam}(\Theta_1))}  \m^{\frac{1}{2\beta_0}}\epsilon^{-(\frac{1}{\beta_0}-1)} \right)^q. 
	$$ 
	Moreover, specify 
	$\eta_2 = \frac{\epsilon^2}{32}$ and by \cite[Lemma A.4]{ghosal2001entropies}, 
	$$
	|\bar{\Lambda}| \leq \left(1+\frac{5}{\eta_2}\right)^{k_0-1}=\left(1+160\epsilon^{-2}\right)^{k_0-1}. 
	$$ Plug the specified $\eta_1$ and $\eta_2$ into \eqref{eqn:Nuppbou1} and the proof is complete.
\end{proof}
	

	\subsection{Minimax lower bounds}
	\label{sec:minimaxlowbou}

	Given $G=\sum_{i=1}^{k_0} p_i \delta_{\theta_i}\in \Ec_{k_0}(\Theta)$ and $G'= \sum_{i=1}^{k_0} p'_i \delta_{\theta'_i} \in \Ec_{k_0}(\Theta)$, define additional notions of distances
	\begin{eqnarray}
	d_{\bm{\Theta}}(G',G):= \min_{\tau\in S_{k_0}}\sum_{i=1}^{k_0}\|\theta'_{\tau(i)}-\theta_i\|_2 \\
	d_{\bm{p}}(G',G):=\min_{\tau\in S_{k_0}}\sum_{i=1}^{k_0}|p'_{\tau(i)}-p_i|. 
	\end{eqnarray}
	Notice that we denote $d_{\Theta}$ to be a distance on $\Theta$ in Section \ref{sec:prelim}. Here the $d_{\bm{\Theta}}$ with bold subscript is on $\Ec_{k_0}(\Theta)$. These two notions of distance are pseudometrics on the space of measures $\Ec_{k_0}(\Theta)$, i.e., they share the same properties as a metric except that allow the distance between two different points be zero. $d_{\bm{\Theta}}(G',G)$ focuses on the distance between atoms of two mixing measure; while $d_{\bm{p}}(G',G)$ focuses on the mixing probabilities of the two mixing measures. It is clear that
	\begin{equation}
	D_N(G,G') \geq \sqrt{N} d_{\bm{\Theta}}(G,G') + d_{\bm{p}}(G,G').
	\label{eqn:d1dthetadp}
	\end{equation}
	

	We proceed to present minimax lower bounds for any sequence of estimators $\hat{G}$, which are measurable functions of $X^1_{[\m]},\ldots, X_{[\m]}^{\n}$, where the sequence length are assumed to be equal for simplicity. The minimax bounds are stated in terms of the aforementioned (pseudo-)metrics $d_{\bm{p}}$ and $d_{\bm{\Theta}}$, as well as the usual metric $D_N$ studied.
	
	\begin{thm}[Minimax Lower Bound] \label{thm:minimaxlower} 
	In the following three bounds the infimum is taken for all $\hat{G} $ measurable functions of $X^1_{[\m]},\ldots, X_{[\m]}^{\n}$.
	\begin{enumerate}[label=\alph*)] 
	\item \label{item:minimaxlowera}	
	Suppose there exists $\theta_0\in\Theta^\circ$ and $\beta_0>0$ such that $\limsup\limits_{\theta \to\theta_0 }\frac{h\left(\P_{\theta},\P_{\theta_0}\right)}{\|{\theta}-{\theta_0}\|_2^{\beta_0}}<\infty$. Moreover, suppose there exists a set of distinct $k_0-1$ points $\{\theta_i\}_{i=1}^{k_0-1}\subset \Theta\backslash \{\theta_0\}$ satisfying 
	$\min_{0\leq i<j\leq k_0-1}h(\P_{\theta_i},\P_{\theta_j})>0$. Then 
	$$
	\inf_{\hat{G}\in \Ec_{k_0}(\Theta)}\sup_{G\in \Ec_{k_0}(\Theta)}\E_{\bigotimes^\n\P_{G,\m}}
	d_{\bm{\Theta}}(\hat{G},G)
	\geq C(\beta_0,k_0) \left(\frac{1}{\sqrt{\n}\sqrt{\m}}\right)^{\frac{1}{\beta_0}},
	$$
	where $C(\beta_0,k_0)$ is a constant depending on $\beta_0$, $k_0$ and the probability family $P_\theta$. 
	\item \label{item:minimaxlowerb} 
	Let $k_0\geq 2$.
	$$\inf_{\hat{G}\in \Ec_{k_0}(\Theta)}\sup_{G\in \Ec_{k_0}(\Theta)}\E_{\bigotimes^\n\P_{G,\m}}
	d_{\bm{p}}(\hat{G},G) \geq C(k_0)\frac{1}{\n},$$
	where $C(k_0)$ is a constant depending on $k_0$ and the probability family $P_\theta$.
    \item 
    Let $k_0\geq 2$. Suppose the conditions of part (a) hold. Then,
    $$\inf_{\hat{G}\in \Ec_{k_0}(\Theta)}\sup_{G\in \Ec_{k_0}(\Theta)}\E_{\bigotimes^\n\P_{G,\m}} D_N(\hat{G},G)\geq C(\beta_0,k_0) \sqrt{N} \left(\frac{1}{\sqrt{\n}\sqrt{\m}}\right)^{\frac{1}{\beta_0}} + C(k_0)\frac{1}{\n}.$$
	\end{enumerate}
	\end{thm}
	%\LN{what is $L_2$ in part (c)?}{\color{purple} (c) is an old version where I make Lipchitz assumption and $L$ is from there. Will be updated.}
	

	\begin{rem} \label{rem:minimax}
	\begin{enumerate}[label=\alph*)]
	 \item 
	The condition that there exists a set of distinct $k_0-1$ points $\{\theta_i\}_{i=1}^{k_0-1}\subset \Theta\backslash \{\theta_0\}$ satisfying 
	$\min_{0\leq i<j\leq k_0-1}h(\P_{\theta_i},\P_{\theta_j})>0$ immediately follows from the injectivity of the map $\theta \mapsto P_\theta$ (recall that this 
	condition is assumed throughout the paper). %The latter is a standard and mild assumption in parameter estimation.
	
	\item The condition that there exists $\theta_0\in\Theta^\circ$ and $\beta_0>0$ such that $\limsup\limits_{\theta \to\theta_0 }\frac{h\left(\P_{\theta},\P_{\theta_0}\right)}{\|{\theta}-{\theta_0}\|_2^{\beta_0}}<\infty$ holds for most probability kernels considered in practice. For example, it is satisfied with $\beta_0=1$ for all full rank exponential families of distribution in their canonical form as shown by Lemma \ref{lem:exphellinger}. It can then be shown that this condition with $\beta_0=1$ is also satisfied by full rank exponential families in general form specified in Corollary \ref{cor:expfamtheta}. Notice that the same remark applies to the condition in Lemma \ref{lem:optimalsquaretootN}.  
	
	
	\item If conditions of Theorem \ref{thm:minimaxlower} \ref{item:minimaxlowera} hold with $\beta_0=1$, then 
	$$
	\inf_{\hat{G}\in \Ec_{k_0}(\Theta)}\sup_{G\in \Ec_{k_0}(\Theta)}\E_{\bigotimes^\n\P_{G,\m}}
	d_{\bm{\Theta}}(\hat{G},G)
	\geq  \frac{C}{\sqrt{\n}\sqrt{\m}}. 
	$$
	That is, the convergence rate of the best possible estimator for the worst scenario is at least  $\frac{1}{\sqrt{\n}\sqrt{\m}}$. Recall that Theorem \ref{thm:posconnotid} implied that the convergence rate of the atoms is $O_P(\sqrt{\frac{\ln(\n N)}{\n N}})$, which is obtained by replacing $\bar{N}_m$ with $N$ in \eqref{eqn:atomconvergencerate}. It is worth noting that while the minimax rate seems to match the posterior contraction rate of the atoms except for a logarithmic factor, such a comparison is not very meaningful as pointwise posterior contraction bounds and minimax lower bounds are generally not considered to be compatible. In particular, in the posterior contraction Theorem \ref{thm:posconiid}, the truth $G_0$ is fixed and the hidden constant $O_P(\sqrt{\frac{\ln(\n N)}{\n N}})$ depends on $G_0$, which is clearly not the case in the above results obtained under the minimax framework. In short, we do not claim that the Bayesian procedure described in Theorem \ref{thm:posconnotid} is optimal in the minimax sense; nor do we claim that the bounds given in Theorem~\ref{thm:minimaxlower} are sharp (i.e., achievable by some statistical procedure). %We leave the resolution of these questions to future study.
	\myeoe
	\end{enumerate}
	\end{rem}
	
	\begin{comment}
	\LN{A question is whether these lower bounds are sharp? Not critical if we don't have a quick answer for it. Yes, that inf =, not $\geq$. I have not thought seriously about this question. Was wondering if you have. It's not very important, though technically interesting. They are of the same spirit, hence equal in significance. But that Lemma is more general, it illustrates a more general phenomenon. I didn't think about the question of tightness of minimax bound under Wr, not because I thought it's hard, but because there were other more pressing questions... I did need the condition that $h/\|\theta-\theta_0\|^2 < \infty$ uniformly in establishing lower bounds. The current minimax results are ok. I'm not sure how to connect it, though. Because they are not compatible. In addition, the bounds are not even the same. In posterior contraction rate we have constant $C(G_0)$, that's the issue. This is where we have to be careful.... not to give misleading claim. The point is, we can't claim optimality in any way. We can only claim whether our bounds are sharp or not. We haven't actually proved that for posterior contraction rates have we. Right, so I think we can add a comment cautioning the reader that the two bounds need not be compatible. That's all we can say. Sounds good.}
	
	\YW{what do you mean sharp? you mean attained by a estimator?Not clear. For all your previous result on minimax, we don't whether it's sharp or not, right? Agree. But I think a) and b) is really what we can say about different minimax convergence rate on atoms and on p. Your previous result on $W_1$ or $W_r$ or $W_r^r$ doesn't tell whether the slow rate is on atom or on p, since it's a lower bound, not upper bound. That's why I write clearly part a) and part b). That's why I think Lemma \ref{lem:VD1r1r2lowbou} is not very important. I prove minimax bound without using those bounds. Ok.My previous comment is not about sharpness. But I think that's not relevant to this paper.}\YW{Another issue is in part (a), I prove it under the assumption limsup, and that is why I suspect that your previous proof might need a limsup condition to hold as well. But again, it's not really relevant in this paper. Do you think the current minimax result is ok?  } \YW{I think we should add some comments after it to connect to posterior contraction, right? True. It's the same, since typical situation is that $\beta_0=1$. Yes, igonore the constant, the bound matches. But they are not copatible I understand. But we should always make some comments after the result, right? No, we don't prove anything about sharpness of posterior contraction. That's why this minimax rate result is awkward. Ok. I can add some comment and maybe you can modify my comments later.}
	\end{comment}
	
		
	\begin{proof}[Proof of Theorem \ref{thm:minimaxlower}]
%	\begin{enumerate}[label=\alph*)]
a) %	\item	
	Choose a set of distinct $k_0-1$ points $\{\theta_i\}_{i=1}^{k_0-1}\subset \Theta\backslash \{\theta_0\}$ satisfying 
	$$\rho_1:=\min_{0\leq i<j\leq k_0-1}h(\P_{\theta_i},\P_{\theta_j})>0.$$ 
	Let $\rho := \min_{0\leq i<j \leq k_0-1}\|\theta_i-\theta_j\|_2$. Since $\limsup\limits_{\theta \to\theta_0 }\frac{h\left(\P_{\theta},\P_{\theta_0}\right)}{\|{\theta}-{\theta_0}\|_2^{\beta_0}}<\infty$, there exist $\gamma\in(0,\infty)$ and $r_0\in(0,\min\{\rho,(\rho_1/\gamma)^{1/\beta_0}\})$ such that 
		\begin{equation}
		\frac{h\left(\P_{\theta},\P_{\theta_0}\right)}{\|{\theta}-{\theta_0}\|_2^{\beta_0}} < \gamma,\quad \forall 0<\|\theta-\theta_0\|_2<r_0. \label{eqn:h2normratioupp}
		\end{equation}
		  Consider $G_1= \sum_{i=1}^{k_0} \frac{1}{k_0} \delta_{\theta_i^1} \in \Ec_{k_0}(\Theta) $ and $G_2= \sum_{i=1}^{k_0} \frac{1}{k_0} \delta_{\theta_i^2} \in \Ec_{k_0}(\Theta)$ with $\theta_i^1=\theta_i^2=\theta_i \in \Theta\backslash\{\theta_0\}$ for $ i\in [k_0-1]$ and $\theta_{k_0}^1=\theta_0$, $\theta_{k_0}^2=\theta$ satisfying $\|\theta-\theta_0\|_2 = 2\epsilon<r_0$. Here $\epsilon\in (0,r_0/2) $ is a constant to be determined. Then $d_{\bm{\Theta}}(G_1,G_2) =2\epsilon$. Moreover, $h(\P_\theta,\P_{\theta_0})\leq \gamma\left(2\epsilon\right)^{\beta_0}<\rho_1$.
		  
		  
		  By two-point Le Cam bound (see \cite[(15.14)]{wainwright2019high})
		\begin{equation}
		\inf_{\hat{G}\in \Ec_{k_0}(\Theta)}\sup_{G\in \Ec_{k_0}(\Theta)}\E_{\bigotimes^\n\P_{G,\m}} d_{\bm{\Theta}}(G,\hat{G})\geq \frac{\epsilon}{2} \left(1- V\left(\bigotimes^\n\P_{G_1,\m}, \bigotimes^\n\P_{G_2,\m}\right) \right).  \label{eqn: minimaxtheta}
		\end{equation}
		Notice 
		$$
		V\left(\bigotimes^\n\P_{G_1,\m}, \bigotimes^\n\P_{G_2,\m}\right)  \leq h\left(\bigotimes^\n\P_{G_1,\m}, \bigotimes^\n\P_{G_2,\m}\right)  \leq \sqrt{\n} h\left(\P_{G_1,\m}, \P_{G_2,\m}\right). 
		$$
		With our choice of $G_1$ and $G_2$, by Lemma \ref{lem:hellingeruppbou}, the last display becomes
		\begin{align*}
		 V\left(\bigotimes^\n\P_{G_1,\m}, \bigotimes^\n\P_{G_2,\m}\right) 
		\leq & \sqrt{\n} \sqrt{\m} \min_{\tau\in S_{k_0}} \max_{1\leq i\leq k_0}   h\left(\P_{\theta^1_i}, \P_{\theta^2_{\tau(i)}}\right) \\
		= & \sqrt{\n} \sqrt{\m} h\left(\P_{\theta_0}, \P_{\theta}\right)\\
		\leq & \sqrt{\n} \sqrt{\m} \gamma \left(2\epsilon\right)^{\beta_0}, \numberthis \label{eqn:minimaxVuppbou}
		\end{align*}
		where the equality follows from $$
		 \min_{\tau\in S_{k_0}} \max_{1\leq i\leq k_0}   h(\P_{\theta^1_i}, \P_{\theta^2_{\tau(i)}})=h(\P_{\theta^1_{k_0}}, \P_{\theta^2_{k_0}}) =  h\left(\P_{\theta_0}, \P_{\theta}\right)
		$$
		due to $h\left(\P_{\theta_0}, \P_{\theta}\right)<\rho_1$. 
		%
		Plug \eqref{eqn:minimaxVuppbou} into \eqref{eqn: minimaxtheta},
		\begin{equation}
		\inf_{\hat{G}\in \Ec_{k_0}(\Theta)}\sup_{G\in \Ec_{k_0}(\Theta)}\E_{\bigotimes^\n\P_{G,\m}} d_{\bm{\Theta}}(G,\hat{G}) \geq \frac{\epsilon}{2} \left(1-\gamma \sqrt{\n} \sqrt{\m} (2\epsilon)^{\beta_0}\right). \label{eqn:minimaxlowboueps}
		\end{equation}
		Consider any $a\in(0,1)$ satisfying $a>1-\gamma r_0^{\beta_0}$ and let $2\epsilon= \left(\frac{1-a}{\gamma\sqrt{\n}\sqrt{\m}}\right)^{\frac{1}{\beta_0}} $. Then $2\epsilon \in (0,r_0)$.  Plug the specified $\epsilon$ into \eqref{eqn:minimaxlowboueps}, then the right hand side in the above display becomes
		$$
	 \frac{a}{4}\left(\frac{1-a}{\gamma\sqrt{\n}\sqrt{\m}}\right)^{\frac{1}{\beta_0}} = C(\beta_0) \left(\frac{1}{\sqrt{\n}\sqrt{\m}}\right)^{\frac{1}{\beta_0}},
		$$
	   where $C(\beta_0)$ depends on $\beta_0$. Notice $a,\gamma,r_0$ are  constants that depends on the probability family $\{\P_\theta\}_{\theta\in \Theta}$ and $k_0$.
		
b) %		\item  
		Consider $k_0>3$. Let $0<\epsilon<(\frac{1}{3}-\frac{1}{3(k_0-2)})/2$ . Consider $G_1= \sum\limits_{i=1}^{2} \frac{1}{3} \delta_{\theta_i} + \sum\limits_{i=3}^{k_0} \frac{1}{3(k_0-2)} \delta_{\theta_i} \in \Ec_{k_0}(\Theta)$ and $G_2=  (\frac{1}{3}-\epsilon)\delta_{\theta_1} + (\frac{1}{3}+\epsilon)\delta_{\theta_2}  + \sum\limits_{i=3}^{k_0} \frac{1}{3(k_0-2)} \delta_{\theta_i} \in \Ec_{k_0}(\Theta)$. By the range of $\epsilon$, $G_2\in \Ec_{k_0}(\Theta)$ and
		 $d_{\bm{p}}(G_1,G_2) =2\epsilon$. Similar to the proof of \ref{item:minimaxlowera}, 
		$$
		\inf_{\hat{G}\in \Ec_{k_0}(\Theta)}\sup_{G\in \Ec_{k_0}(\Theta)}\E_{\bigotimes^\n\P_{G,\m}} d_{\bm{p}}(\hat{G},G) \geq \frac{\epsilon}{2} \left(1- \sqrt{\n} h\left(\P_{G_1,\m}, \P_{G_2,\m}\right) \right).
		$$
		With our choice of $G_1$ and $G_2$, by Lemma \ref{lem:hellingeruppbou}, 
		$$
		 h\left(\P_{G_1,\m}, \P_{G_2,\m}\right) \leq \sqrt{\frac{1}{2}\times 2\epsilon}=\sqrt{\epsilon}.
		$$
		Combining the last two displays,
		$$\inf_{\hat{G}\in \Ec_{k_0}(\Theta)}\sup_{G\in \Ec_{k_0}(\Theta)}\E_{\bigotimes^\n\P_{G,\m}} d_{\bm{p}}(\hat{G},G)\geq \frac{\epsilon}{2} \left(1- \sqrt{\n} \sqrt{\epsilon} \right).$$
		The proof is complete by specifying $\epsilon =  \frac{1}{\n} (\frac{1}{3}-\frac{1}{3(k_0-2)})/4 <(\frac{1}{3}-\frac{1}{3(k_0-2)})/2$. The case for $k_0=2$ and $k_0=3$ follow similarly. 
		
c) %		\item 
		The proof follows from \ref{item:minimaxlowera},  \ref{item:minimaxlowerb} and ~\eqref{eqn:d1dthetadp}.
%		\end{enumerate}
	\end{proof}
	



